Fast Generation of Big Random Binary Trees

random_tree() is a linear time and space C++ implementation able to create trees of up to a billion nodes for genetic programming and genetic improvement experiments. A 3.60GHz CPU can generate more than 18 million random nodes for GP program trees per second.

==> author.tex <==
%WBL 13 Jan 2020 Added to bigtree.tex for bugfix 1.1 $Revision: 1.1 $

\centerline{\large \itshape W. B. Langdon}\\[5ex]

\centerline{
\begin{tabular}{lll}
Revision 1.0 & 10 Jan 2020 & Released\\
Revision 1.1 & 13 Jan 2020 & Correct Figure 1\\
\end{tabular}
}

